You Only Prune Once: Designing Calibration-Free Model Compression With Policy Learning

The ever-increasing size of large language models (LLMs) presents significant challenges for deployment due to their heavy computational and memory requirements. Current model pruning techniques attempt to alleviate these issues by relying heavily on external calibration datasets to determine which parameters to prune or compress, thus limiting their flexibility and scalability across different compression ratios. Moreover, these methods often cause severe performance degradation, particularly in downstream tasks, when subjected to higher compression rates. In this paper, we propose PruneNet, a novel model compression method that addresses these limitations by reformulating model pruning as a policy learning process. PruneNet decouples the pruning process from the model architecture, eliminating the need for calibration datasets. It learns a stochastic pruning policy to assess parameter importance solely based on intrinsic model properties while preserving the spectral structure to minimize information loss. PruneNet can compress the LLaMA-2-7B model in just 15 minutes, achieving over 80% retention of its zero-shot performance with a 30% compression ratio, outperforming existing methods that retain only 75% performance. Furthermore, on complex multitask language understanding tasks, PruneNet demonstrates its robustness by preserving up to 80% performance of the original model, proving itself a superior alternative to conventional structured compression techniques.

==> extreme_sparsity_results.tex <==
% Table generated by Excel2LaTeX from sheet 'generative_comparison'
\begin{table}[!t]
  \centering
  \scalebox{0.75}{
    \begin{tabular}{clccc}
    \cline{1-5}
    \multicolumn{1}{l}{\bf Comp. Ratio} & \textbf{Method} & \multicolumn{1}{l}{\textbf{PIQA}} & \multicolumn{1}{l}{\textbf{Hellaswag}} & \multicolumn{1}{l}{\textbf{Average}} \\
    \cline{1-5}
    \multirow{1}[0]{*}{0\%} & Dense & 77.91 & 71.26 & 74.58 \\
    \cdashline{1-5}
    \multirow{5}[0]{*}{30\%} & \modelname & 71.11 & \bf 58.30 & \bf 64.70 \\
     & LLM Pruner~\citep{ma2023llm}$\dagger$  & \bf 71.22 & 56.46 & 63.84\\
          & SliceGPT~\citep{ashkboos2024slicegptcompresslargelanguage}$\dagger$  & 66.21 & 50.27 & 58.24 \\
          & LaCo~\citep{yang2024lacolargelanguagemodel}$\dagger$   & 69.80  & 55.69 & 62.74 \\
          & ShortGPT~\citep{men2024shortgptlayerslargelanguage}$\dagger$  & 66.43 & 53.02 & 59.72 \\
    \cline{1-5}
    \end{tabular}%
    }
    \caption{Comparison of different model compression methods on generative tasks with the LLaMA-2-7B model without recovery fine-tuning. Results marked with `$\dagger$' are taken from ~\cite{men2024shortgptlayerslargelanguage}.}
      \label{tab:extreme_results}%
\end{table}%


==> rebuttal/ZGwt.tex <==
\section*{Reviewer ZGwt}

%\noindent \ZG{This is the color for reviewer ZGwT.}

\noindent \textbf{Structural interdependencies with subsequent layers.} We argue that the interdependencies between subsequent layers are already captured during the pre-training phase of the LLM. Therefore, the spectral structure of the feedforward layers already preserves the information propagation between the subsequent layers. By preserving the spectral structure after compression, \modelname\ preserves the information that needs to be maintained at later layers, therefore omitting additional effort to preserve the information flow between interconnected layers. 
\newline

\noindent \textbf{A comparison with simple random sampling and the efficiency of policy-learning for pruning.} We highlight the results with random policy in Table~\ref{tab:random_policy}, where we select the pruned indices randomly for each model parameter. We refer to this as a 'random' selection. We observe an average $2\%$ drop with a random selection method, demonstrating the need for a learnable policy for effective model compression. \\
Moreover, Table~\ref{tab:diff_policy} highlights the results with LLaMA-2-7B with deterministic and stochastic (policy learned with \modelname) policies. In the deterministic policy, we chose only the topk (k depends on the compression ratio) parameters based on the importance metric defined in Equation 3. We observe that deterministic policy often underperforms the stochastic policy with an average margin of $4\%$. The results highlight that learnable parameters alone are insufficient to determine which ones to compress. Preserving the spectral structure between the compressed and uncompressed models is also critical to ensure minimal performance drop post-compression.\newline

\noindent \textbf{Efficacy of \texttt{PruneNet} on larger models.} In Table~\ref{llama_13b_results} we highlight the results with \modelname\ and SliceGPT for different compression ratios for LLaMA-2-13B model. For larger models like LLaMA-13B, at a high compression ratio, the performance drops drastically. However, the results in Table~\ref{llama_13b_results_with_rft} highlight that after recovery fine-tuning, the compressed models regain the performance quickly and can preserve up to $84\%$ of the original uncompressed model performance, even at a high compression rate of $30\%$. \modelname\ also outperforms SliceGPT with a margin of $2\%$, showcasing a similar trend as the smaller LLMs used in our study.\newline

==> rebuttal/bk7b.tex <==
\section*{Reviewer bk7b}

%\noindent \bk{This is the color for reviewer bk7b.}

\noindent \textbf{Comparison with SliceGPT with Alpaca calibration data.} Table \ref{alpaca_without_rft} contains a comparison of the performance of the LLaMA-2-7B and Phi-2 pruned with SliceGPT using the Alpaca calibration dataset (as opposed to the WikiText2 dataset, used in the main text of our paper). While LLaMA-2-7B pruned with SliceGPT exhibits better average performance for all compression ratios, Phi-2 exhibits an opposite trend, wherein \modelname\ beats SliceGPT by a consistent margin of at least $2\%$ for all compression ratios. This trend reinforces a fundamental limitation of calibration data-based pruning techniques~\citep{anonymous2024beware}, namely their sensitivity to the choice and quality of the calibration dataset and the choice of model architectures. In conjunction with this, it should also be noted that the Alpaca dataset is an instruction-tuning dataset (as opposed to WikiText2). Therefore, it is not unreasonable for the performance of pruned models calibrated with the Alpaca dataset on generative tasks to be better than a calibration-free technique like \modelname. \newline

\noindent \textbf{Motivation for calibration-free model compression techniques.} While it is true that there is an abundance of calibration data for textual modalities, it is not the \textit{availability} of calibration data alone that determines the quality of a pruned model. A detailed study by \citep{Williams_2024} reveals a large degree of sensitivity in the performance on downstream tasks of pruned models based on the selected calibration data and model architectures, which questions the usability of calibration-based pruning methods in data-private settings; this has made the problem of sampling high-quality calibration datasets an active area of model pruning research. Another major limitation of calibration-based pruning techniques is that of \textit{reusability}, wherein pruning multiple models necessitates running the forward/backward passes of pruned models on the calibration datasets, making the overall process highly inefficient. In contrast, \modelname\ aims to be the \textit{first} pruning technique to alleviate these difficulties and can also run right out of the box in low-resource/compute settings. Finally, \modelname\ can be used in data modalities other than text, where sampling calibration data might be costly. \newline

\noindent \textbf{Justification of spectrum matching and comparison with other reward criterion.} It is important to understand that pruning reduces the cardinality of the spectrum. Therefore, the traditional pointwise distance measures (like Euclidean/Cosine/Frobenius norm) are not applicable for comparing the spectrum structure of uncompressed and compressed models. Therefore, we resort to probabilistic distance measures that can capture the shift in the empirical distribution of spectrums of the compressed model. Corollary 3.3 suggests that compression reduces the spectrum range, and Figure 1 highlights that with more compression, the spectrum becomes more right-skewed. To further understand the effectiveness of \modelname\ under different distance measures, we evaluate the LLaMA-2-7B model compressed using \modelname\ with non-parametric Anderson–Darling measure of agreement. Table~\ref{tab:other_loss_policy} highlights the effectiveness of \modelname\ with both Kolmogorov-Smirnov (highlighted as KS) and  Anderson–Darling (highlighted as AD) distance measures. Under both reward functions, we observe a similar performance of \modelname\ for different compression ratios with the LLaMA-2-7B model. The results further emphasize the stability of our proposed compression method under different choice metrics. \newline

\subsection{Follow up questions}

\noindent \textbf{Discrepancy in the tables.} The only discrepancy between the table above for the performance of SliceGPT on Phi-2 and the one given in Table 8 of the original paper (\cite{ashkboos2024slicegptcompresslargelanguage}) is the average accuracy on all tasks with a compression ratio of 30\%; the SliceGPT authors have reported an incorrect number, and our table contains the correct result. We agree that including results with the Alpaca dataset is important, and we've done so in the updated version of the paper.\newline

\noindent \textbf{On RFT and calibration data.} We again emphasize on the fact that a careful selection of calibration dataset, which may require extensive experimentation, is in itself a major limitation of such methods and may not be readily applicable in all model compression settings. For instance, consider a scenario where an LLM has been trained on private data to be used in domain-specific applications such as those related to healthcare or medicine. In such a situation, even finding good quality calibration datasets might be monetarily and legally demanding. \newline

\noindent Another point which motivated us to pursue data-free pruning methods was the fact that calibration-based pruning methods perform computation in the model space, which require loading the calibration data in memory and running it through the model. This requirement will not be suitable in low-resource/compute scenarios; for instance, an end user may want to compress a vision LLM tailored to video data. \modelname\ is akin to usual quantization methods in this regard, which don't require heavy activation/gradient based computations on datasets (which has also led to many users to prefer quantization methods over calibration-based pruning techniques to compress models). This also makes \modelname\ more efficient compared to methods such as SliceGPT in terms of time complexity, wherein our method can potentially be twice as faster. \newline

\noindent \textbf{On spectrum matching.} Observe that the key operation performed by \modelname\ is the \textit{slicing} of matrices. To gain some insight into the overall effect of slicing on the spectrum of a matrix, we proved \textbf{Corollary 3.3}, which proved that slicing a matrix shrinks it's spectrum range. We used this as a basis to design our penalty-based objective of \modelname. To understand the importance of using a learned policy, we further carried out the following experiment: we randomly pick indices to slice off for each layer, and report the standard deviation and mean of the obtained rewards.

==> rebuttal/onBH.tex <==
\section*{Reviewer obBH}

%\noindent \on{This is the color for reviewer onBH.}

\noindent \textbf{A comparison of pruning on FFN1 vs FFN2 layers.} Table~\ref{ffn1_vs_ffn2} highlights the zero-shot performance of LLaMA-2-7B model compressed with \modelname\ with policy learned on different FFN matrices. In most cases, we observe marginal differences in the result ($< 1\%$) when the policy is learned with FFN2 instead of FFN1. The observations emphasize that \modelname\ is invariant to the choice of parameter used for learning the policy. \newline

\noindent \textbf{Usage of reward functions other than the KS distance.} It is important to notice that compression reduces the cardinality of the spectrum. Therefore, the traditional pointwise distance measures (like Euclidean/Cosine/Frobenius) are not applicable for comparing the distance between the spectrum structure of uncompressed and compressed models. Therefore, we resort to probabilistic distance measures that can capture the shift in distribution structures of the compressed model. \\
To further understand the effectiveness of \modelname\ under different distance measures, we evaluate the LLaMA-2-7B model compressed using \modelname\ with non-parametric Anderson–Darling measure of agreement. Table~\ref{tab:other_loss_policy} highlights the effectiveness of \modelname\ with both Kolmogorov-Smirnov (highlighted as KS) and  Anderson–Darling (highlighted as AD) distance measures. Under both reward functions, we observe a similar performance of \modelname\ for different compression ratios with the LLaMA-2-7B model. The results further emphasize the stability of our proposed compression method under different choice metrics. \newline

\noindent \textbf{Motivation behind the usage of discounted rewards and singular values of deeper layers.} Weight matrices of LLMs have been known to exhibit a variation in the distribution of singular values across layers \citep{yuan2024asvdactivationawaresingularvalue}. To further verify our observations from Figure 1 of the main text, we conduct a similar study on the FFN1 matrices of the OPT and Phi-2 models. We plot the cumulative distribution of the singular values of these matrices and observe consistent behaviour across all three model architectures. Figure~\ref{fig:phi_spectrum} and~\ref{fig:opt_spectrum} highlights the spectrum of the FFN1 module at different layers for Phi-2 and OPT-2.7B models, respectively. This further strengthens our assumption of using discounted rewards in our policy learning approach. 
\newline

\begin{figure}
    \centering
    \subfloat[Phi-2]{\includegraphics[width=0.5\linewidth]{images/motivation_phi.pdf}
    \label{fig:phi_spectrum}}
    \subfloat[OPT-2.7B]{\includegraphics[width=0.5\linewidth]{images/motivation_opt.pdf}
    \label{fig:opt_spectrum}}
    \caption{Spectrum of FFN1 layer for Phi-2 (a) and OPT-2.7B (b) models at different compression ratios.}
\end{figure}

\noindent \textbf{Detailed results of the one-sided KS test.} For LLaMA-2-7B and Phi-2 models, we calculate the recovered performance ($\frac{\text{Compressed model performance}}{\text{Dense model performance}}$) for different compression ratios with \modelname\ and SliceGPT. We conduct a one-sided KS test with the null hypothesis as SliceGPT recovered performance higher than \modelname\ recovered performance for different compression ratios. For compression ratio $20\%$, we obtain the test statistics value of 0.5 and $p$-value $0.043$, suggesting us to reject the null hypothesis. Similarly, for compression ratio $25\%$ and $30\%$ we obtain statistics $0.5$ ($p$-value $0.043$) and $0.6$ ($p$-value $0.026$), respectively. With these statistical results, we conclude that the performance recovered with \modelname\ is higher than SliceGPT with statistical significance. \newline

\noindent \textbf{Why does RFT \textit{reduce} performance of models like Phi2?} Although interpreting the performance of a model compression method requires much detailed analysis, which is much out of scope for our current study, we can make certain educated guesses to understand the behaviours of different LLMs under compression. One possible reason behind the inferior performance of Phi-2 under RFT could be attributed to its pre-training objective. Phi-2 is pre-trained on a vast amount of synthetic texts~\cite {li2023textbooks}, which allows it to perform reasonably well on common sense and logical reasoning tasks (the tasks used in our work) even without fine-tuning. Therefore, fine-tuning on additional datasets like WikiText2 or Alpaca could hurt the model's performance. Table 2 of the paper shows that the post-compression Phi-2 model demonstrates higher performance recovery than any other LLM, indicating its robustness on complex reasoning tasks, even after compression. Unlike SliceGPT, \modelname\ preserves the original knowledge base of LLMs by preserving spectral structures. Therefore, additional fine-tuning can distort the reasoning abilities of the compressed LLM, adversely affecting its zero-shot performance. \newline

\noindent \textbf{A comparison of \texttt{PruneNet} with SliceGPT with RFT.} We report the results with LLaMA-2-7B with RFT on Wikitext2 and Alpaca datasets in Table~\ref{wikitext_with_rft} and Table~\ref{alpaca_with_rft}, respectively. With RFT on Wikitext2 dataset, \modelname\ achieves on average $>5\%$ accuracy than SliceGPT. However, SliceGPT outperforms \modelname\ when fine-tuned on the Alpaca dataset, with an average margin of $3\%$. As SliceGPT uses the same datasets for calibration and RFT, it typically has access to more instruction-tuning datasets than \modelname\, allowing it to do better when fine-tuned on the Alpaca dataset. However, it is worth noticing that the average standard deviation in the performance of SliceGPT after RFT is significantly high ($5.5$), compared to \modelname\ ($1.5$). The low standard deviation highlights the robustness of \modelname\ when fine-tuned on different datasets for recovering the information loss during compression.
\newline

\noindent \textbf{An implementation of policy-based pruning for attention layers.} We carry out a similar pruning strategy on attention layers, wherein we learn importance scores of the rows for the \textit{output matrix} of the attention layer, and correspondly slice off the key, query and value matrices to keep the output dimension consistent. We highlight the pruning results for LLaMA-2-7B model with compressed self-attention layers in Table~\ref{attention_slicing}. The performance drop with the compressed models suggests that compressing self-attention layers intrinsically is harder than compressing FFN layers. However, around $50\%$ of the performance drop can be recovered with recovery fine-tuning.
\newline

\noindent \textbf{Performance drops for \texttt{PruneNet} with high compression ratios ($>40\%$).} Table~\ref{high_compression} highlights the performance of LLaMA-2-7B model at $50\%$ compression ratio with \modelname\ and SliceGPT. While both the construct can regain only $60\%$ of the performance of the original uncompressed model, \modelname\ demonstrates $2\%$ better than the SliceGPT, showcasing its effectiveness over the baseline, even at a very high compression rate.\newline

==> rebuttal/ooUI.tex <==
\section*{Reviewer ooUI}

%\noindent \oo{This is the color for reviewer ooUI.}

\noindent \textbf{Comparison of \texttt{PruneNet} with other compression methods with RFT enabled.} We report the results with LLaMA-2-7B with RFT on Wikitext2 and Alpaca datasets in Table~\ref{wikitext_with_rft} and Table~\ref{alpaca_with_rft}, respectively. With RFT on Wikitext2 dataset, \modelname\ achieves on average $>5\%$ accuracy than SliceGPT. However, SliceGPT outperforms \modelname\ when fine-tuned on the Alpaca dataset, with an average margin of $3\%$. As SliceGPT uses the same datasets for calibration and RFT, it typically has access to more instruction-tuning datasets than \modelname\, allowing it to do better when fine-tuned on the Alpaca dataset. However, it is worth noticing that the average standard deviation in the performance of SliceGPT after RFT is significantly high ($5.5$) compared to \modelname\ ($1.5$). The low standard deviation highlights the robustness of \modelname\ when fine-tuned on different datasets for recovering the information loss during compression.\newline

\noindent \textbf{Efficiency of policy learning.} The primary motivation behind policy learning is to decouple the model pruning process from the model itself. Therefore, with an appropriate policy learner model, we can learn which parameters can be compressed within an arbitrary model component just by looking at the model parameters without posing any additional constraint on the component architecture. This allows us to flexibly use the same policy learner model for compressing different layers and components of an LLM. \\
To further understand the effectiveness of the learned policy empirically, we perform experiments where we learn deterministic policy based on the parameter importance calculated in Equation 3 of the paper. In the deterministic policy, we chose only the topk parameters based on this computed importance metric, making the selection deterministic. Table~\ref{tab:random_policy} highlights the results with LLaMA-2-7B with deterministic and stochastic (policy learned with \modelname defined in Equation 5 of the paper) policies. We observe that deterministic policy often underperforms the stochastic policy with an average margin of $2\%$. The results highlight that parameter importance alone cannot determine which parameters to compress. Preserving the spectral structure between the compressed and uncompressed models is also critical to ensure minimal performance drop post-compression.\newline

\noindent \textbf{Computational budget.} The policy learner model is typically $1000$ times smaller than the LLM to be compressed (number of learnable parameters $<7$M). As Section 1 of the paper highlights, most existing structured pruning methods learn the compressed model after being calibrated on some dataset. Therefore, the computational budget utilized by the policy learner model is far less than the existing baselines, making our compression method more scalable and efficient. \newline

\noindent \textbf{Pseudo code.} We thank the reviewer for the suggestion. We have added the pseudo-code of the proposed compression method in Algorithm~\ref{alg:prunenet}.\newline

\input{algorithm}

\noindent \textbf{A detailed motivation behind design choices.} The key motivation behind the design of \modelname\ is to have a predictor network which can compute the importance scores of the rows of \textit{any} weight matrix; this allows us to reuse the same learned predictor network to prune the FFN weight matrix of \textit{any} layer in the model, which turns out to be extremely efficient compared to other SOTA pruning methods.\newline 

\noindent Some clarification about equation (3) of main text is in order. Note that the output of equation (3) is an $n$-dimensional vector (and not a $d$-dimensional vector), where $n$ is the number of rows in the weight matrix $W$. In essence, the predictor network is computing importance scores for each row of a weight matrix in two steps: in the first part of equation (3), the network computes the \textit{relative importance} of rows amongst themselves. This is needed since the importance of a row is potentially correlated with the importance of other rows of the weight matrix. The second part of equation (3), particularly the matrix multiplication within $\sigma$, simply projects the $n\times n$ matrix of relative importance scores into an output vector of importance scores of each row. In contrast, as suggested by the reviewer, directly optimizing a vector of importance scores conflicts with our design philosophy of \textit{reusability} of the learned predictor network. Please see part 2 of our rebuttal for reviewer bk7b for a motivation behind our usage of a distributional distance measure, and a comparison of different reward criterion for the policy learning process.\newline

\noindent We further perform an ablation study to understand the importance of different components of \modelname. \newline

\noindent We conduct experiments with a random selection process, where the pruned parameter indices are chosen randomly. We highlight the results with random policy in Table~\ref{tab:random_policy}. We observe an average $2\%$ drop with a random selection method, justifying the need to learn which parameters to compress for more effective model compression.\\
Table~\ref{tab:diff_policy} highlights the results with LLaMA-2-7B with deterministic and stochastic (policy learned with \modelname in Equation 5 of the paper) policies.  In the deterministic policy, we chose only the topk parameters based on the importance metric defined in Equation 3. We observe that deterministic policy often underperforms the stochastic policy with an average margin of $4\%$. The results highlight that parameter importance alone cannot determine which parameters to compress. Preserving the spectral structure between the compressed and uncompressed models is critical to ensure minimal performance drop post-compression. \\
To further understand the effectiveness of \modelname\ under different distance measures, we evaluate the LLaMA-2-7B model compressed using \modelname\ with non-parametric Anderson–Darling measure of agreement. Table~\ref{tab:other_loss_policy} highlights the effectiveness of \modelname\ with both Kolmogorov-Smirnov (highlighted as KS) and  Anderson–Darling (highlighted as AD) distance measures. Under both reward functions, we observe a similar performance of \modelname\ for different compression ratios with the LLaMA-2-7B model. The results further emphasize the stability of our proposed compression method under different choice metrics.\\
Table~\ref{ffn1_vs_ffn2} highlights the zero-shot performance of the LLaMA-2-7B model compressed with \modelname\ with policy learned on different FFN matrices. In most cases, we observe marginal differences in the result ($< 1\%$) when the policy is learned with FFN2 instead of FFN1. The observations emphasize that \modelname\ is invariant to the choice of parameter used for learning the policy. \newline

\noindent \textbf{Question.} We explained above that directly optimizing the parameter importance often leads to poorer performance than the learned compression policy. We reuse the same policy learner for all the layers within the LLM. The policy learner is agnostic to the model architecture and learns a mapping between the compressed and uncompressed model parameters. The simplicity of the policy learner allows us to reuse the same model to compress an LLM at any given compression ratio, offering greater flexibility and efficiency.




==> rft_dataset_llama.tex <==
% Table generated by Excel2LaTeX from sheet 'different_dataset'
\begin{table}
  \centering
  \scalebox{0.7}{
    \begin{tabular}{clrrrrrr}
    \cline{1-8}
    \multicolumn{1}{l}{\textbf{Comp. Ratio}} & \textbf{RFT Dataset} & \multicolumn{1}{l}{\textbf{PIQA}} & \multicolumn{1}{l}{\textbf{WinoGrande}} & \multicolumn{1}{l}{\textbf{HellaSwag}} & \multicolumn{1}{l}{\textbf{ARC-e}} & \multicolumn{1}{l}{\textbf{ARC-c}} & \multicolumn{1}{l}{\textbf{Average}} \\
    \cline{1-8}
    %\multirow{3}[0]{*}{10\%} & Alpaca & 77.31 & 68.82 & 72.09 & 66.04 & 43.17 & 65.49 \\
    %      & PTB   & 75.95 & 65.98 & 70.02 & 70.12 & 41.72 & 64.76 \\
    %      & WikiText2 & 76.88 & 67.64 & 72.86 & 71.30 & 43.86 & 66.51 \\
    %\cdashline{1-8}
    \multirow{3}[0]{*}{20\%} & Alpaca & 72.73 & 62.25 & 66.45 & 61.52 & 42.15 & 61.02 \\
          & PTB   & 73.07 & 63.38 & 65.05 & 64.56 & 36.69 & 60.55 \\
          & WikiText2 & 74.76 & 66.22 & 69.38 & 65.61 & 39.25 & 63.04 \\
    \cdashline{1-8}
    \multirow{3}[0]{*}{25\%} & Alpaca & 75.79 & 62.35 & 65.48 & 60.94 & 39.16 & 60.74 \\
          & PTB   & 73.47 & 63.28 & 63.56 & 62.79 & 36.19 & 59.86 \\
          & WikiText2 & 74.37 & 66.46 & 65.71 & 60.82 & 36.60 & 60.79 \\
    \cdashline{1-8}
    \multirow{3}[0]{*}{30\%} & Alpaca & 72.14 & 62.75 & 62.38 & 55.43 & 37.03 & 57.95 \\
          & PTB   & 71.11 & 62.67 & 59.60 & 58.12 & 35.07 & 57.31 \\
          & WikiText2 & 73.01 & 63.46 & 63.21 & 60.14 & 35.92 & 59.15 \\
    \cline{1-8}
    \end{tabular}%
    }
    \caption{Results obtained by LLaMA-2-7B after recovery finetuning on Alpaca, PTB and WikiText2 datasets with different compression ratios.}
      \label{tab:rft_datasetwise_llama}%
      \vspace{-5mm}
\end{table}%


==> tables/all_results_with_RFT.tex <==
% Table generated by Excel2LaTeX from sheet 'all_results_with_RFT'
\begin{table}[htbp]
  \centering
    \begin{tabular}{ccrrrrrr}
    \cline{1-8}
    \textbf{Model} & \textbf{Comp. Ratio} & \textbf{PIQA} & \textbf{WinoGrande} & \textbf{HellaSwag} & \textbf{ARC-e} & \textbf{ARC-c} & \textbf{Average} \\
    \cline{1-8}
        %\multirow{2}[0]{*}{OPT-125M} & 10\%  & 60.88 & 51.54 & 30.38 & 37.21 & 23.21 & 40.64 \\
        \multirow{3}[0]{*}{OPT-125M}   & 20\%  & 60.01 & 50.59 & 30.17 & 35.23 & 22.95 & 39.79 \\
          & 25\%  & 59.54 & 48.81 & 30.02 & 34.92 & 22.07 & 39.07 \\
           & 30\%  & 59.01 & 47.90 & 29.87 & 34.26 & 21.54 & 38.52 \\
        \cdashline{1-8}
    %\multirow{4}[0]{*}{OPT-2.7B} & 10\%  & 69.91 & 57.54 & 52.81 & 46.13 & 29.01 & 51.08 \\
         \multirow{3}[0]{*}{OPT-2.7B} & 20\%  & 70.02 & 58.33 & 50.52 & 46.30 & 27.73 & 50.58 \\
          & 25\%  & 68.88 & 57.46 & 47.91 & 45.83 & 27.82 & 49.58 \\
          & 30\%  & 66.21 & 56.99 & 46.61 & 43.56 & 27.05 & 48.08 \\
    \cdashline{1-8}
    %\multirow{4}[0]{*}{OPT-6.7B} & 10\%  & 73.61 & 62.19 & 62.41 & 51.14 & 32.51 & 56.37 \\
     \multirow{3}[0]{*}{OPT-6.7B}     & 20\%  & 72.80 & 61.64 & 59.08 & 49.49 & 31.06 & 54.81 \\
          & 25\%  & 72.69 & 60.38 & 57.01 & 48.61 & 30.38 & 53.81 \\
          & 30\%  & 70.84 & 58.25 & 55.50 & 46.93 & 29.95 & 52.29 \\
    \cdashline{1-8}
    %\multirow{4}[0]{*}{LLaMA-2-7B} & 10\%  & 76.88 & 67.64 & 72.86 & 71.30 & 43.86 & 66.51 \\
     \multirow{3}[0]{*}{LLaMA-2-7B}     & 20\%  & 74.76 & 66.22 & 69.38 & 65.61 & 39.25 & 63.04 \\
          & 25\%  & 74.37 & 66.46 & 65.71 & 60.82 & 36.60 & 60.79 \\
          & 30\%  & 73.01 & 63.46 & 63.21 & 60.14 & 35.92 & 59.15 \\
    \cdashline{1-8}
    %\multirow{4}[0]{*}{Phi-2} & 10\%  & 77.37 & 74.74 & 68.85 & 75.55 & 51.45 & 69.59 \\
       \multirow{3}[0]{*}{Phi-2}   & 20\%  & 76.17 & 71.51 & 63.28 & 70.50 & 46.42 & 65.58 \\
          & 25\%  & 73.39 & 69.22 & 61.53 & 71.38 & 45.73 & 64.25 \\
          & 30\%  & 71.49 & 63.93 & 58.18 & 61.78 & 37.80 & 58.64 \\
    \cdashline{1-8}
    %\multirow{4}[0]{*}{Phi-2} & 10\%  & 77.37 & 74.74 & 68.85 & 75.55 & 51.45 & 69.59 \\
       \multirow{3}[0]{*}{LLaMA-1-7B}   & 20\%  & 76.17 & 71.51 & 63.28 & 70.50 & 46.42 & 65.58 \\
          & 25\%  & \\
          & 30\%  &  \\
    \cline{1-8}
    \end{tabular}%
        \caption{Zero-shot performance of compressed LLMs after recovery fine-tuning on the WikiText2 dataset.}
  \label{tab:all_results_with_rft}%
\end{table}%


==> tables/mmlu_with_rft.tex <==
% Table generated by Excel2LaTeX from sheet 'temp'
\begin{table}[htbp]
  \centering
  \scalebox{0.65}{
    \begin{tabular}{ccrrrrrrrrrrr}
    \cline{1-13}
    \textbf{Model} & \textbf{Comp. Ratio} & \multicolumn{1}{l}{\textbf{Abs. Alg.}} & \multicolumn{1}{l}{\textbf{Bus. Eth.}} & \multicolumn{1}{l}{\textbf{Clg. CS.}} & \multicolumn{1}{l}{\textbf{Clg. Math}} & \multicolumn{1}{l}{\textbf{Con. Phy.}} & \multicolumn{1}{l}{\textbf{Frm. Log.}} & \multicolumn{1}{l}{\textbf{Glb. Fct.}} & \multicolumn{1}{l}{\textbf{ML.}} & \multicolumn{1}{l}{\textbf{Misc.}} & \multicolumn{1}{l}{\textbf{Phil.}} & \multicolumn{1}{l}{\textbf{MMLU Avg.}} \\
    \cline{1-13}
    \multirow{2}[0]{*}{\rotatebox[origin=c]{90}{OPT-125M}} & 10\%  & 21    & 30    & 24    & 21    & 26.4  & 25.4  & 18    & 30.4  & 23.5  & 18.6  & 23.8 \\
          & 20\%  & 22    & 30    & 26    & 21    & 26.4  & 28.6  & 18    & 32.1  & 23.6  & 18.6  & 24.6 \\
    \cdashline{1-13}
    \multirow{4}[0]{*}{\rotatebox[origin=c]{90}{OPT-2.7B}} & 10\%  & 22    & 26    & 29    & 19    & 25.1  & 29.4  & 23    & 29.5  & 27    & 18.3  & 24.8 \\
          & 20\%  & 22    & 24    & 24    & 21    & 24.7  & 29.4  & 24    & 25.9  & 25    & 20.6  & 24.1 \\
          & 25\%  & 22    & 30    & 25    & 21    & 26    & 28.6  & 18    & 31.2  & 24.1  & 18.6  & 24.4 \\
          & 30\%  & 22    & 30    & 26    & 21    & 26    & 27.8  & 18    & 31.2  & 23.6  & 18.6  & 24.4 \\
    \cdashline{1-13}
    \multirow{4}[0]{*}{\rotatebox[origin=c]{90}{OPT-6.7B}} & 10\%  & 23    & 25    & 34    & 32    & 21.3  & 23    & 24    & 34.8  & 27.8  & 19.3  & 26.4 \\
          & 20\%  & 30    & 27    & 24    & 27    & 21.3  & 17.5  & 32    & 23.2  & 26.8  & 28.3  & 25.7 \\
          & 25\%  & 22    & 30    & 30    & 23    & 28.9  & 23    & 20    & 29.5  & 26.7  & 17.7  & 25.1 \\
          & 30\%  & 29    & 23    & 28    & 23    & 20.8  & 21.4  & 25    & 19.6  & 25    & 21.2  & 23.6 \\
    \cdashline{1-13}
    \multirow{4}[0]{*}{\rotatebox[origin=c]{90}{LLaMA-2-7B}} & 10\%  & 28    & 36    & 34    & 33    & 34    & 35.7  & 36    & 35.7  & 44.1  & 43.1  & 36 \\
          & 20\%  & 30    & 43    & 31    & 33    & 30.2  & 30.2  & 27    & 32.1  & 35.6  & 33.1  & 32.5 \\
          & 25\%  & 23    & 31    & 33    & 27    & 27.7  & 30.2  & 19    & 31.2  & 32.7  & 28.3  & 28.3 \\
          & 30\%  & 24    & 29    & 38    & 33    & 26.4  & 35.7  & 33    & 32.1  & 26.4  & 29.3  & 30.7 \\
    \cdashline{1-13}
    \multirow{4}[0]{*}{\rotatebox[origin=c]{90}{Phi-2}} & 10\%  & 24    & 54    & 31    & 29    & 40    & 27    & 34    & 35.7  & 59.9  & 50.2  & 38.5 \\
          & 20\%  & 24    & 51    & 37    & 31    & 35.3  & 26.2  & 29    & 33    & 61.2  & 46.3  & 37.4 \\
          & 25\%  & 28    & 37    & 26    & 35    & 39.2  & 26.2  & 35    & 27.7  & 55.4  & 45.3  & 35.5 \\
          & 30\%  & 22    & 41    & 32    & 27    & 30.6  & 27    & 22    & 26.8  & 39.6  & 26    & 29.4 \\
    
        \cline{1-13}
    \end{tabular}%
    }
    \caption{Zero-shot performance of compressed LLMs on MMLU tasks after recovery finetuning on WikiText2 dataset.}
  \label{tab:mmlu_with_rft}%
\end{table}%
